Ultra-Range Gesture Recognition using a Web-Camera in Human-Robot Interaction

Hand gestures play a significant role in human interactions where non-verbal intentions, thoughts and commands are conveyed. In Human-Robot Interaction (HRI), hand gestures offer a similar and efficient medium for conveying clear and rapid directives to a robotic agent. However, state-of-the-art vision-based methods for gesture recognition have been shown to be effective only up to a user-camera distance of seven meters. Such a short distance range limits practical HRI with, for example, service robots, search and rescue robots and drones. In this work, we address the Ultra-Range Gesture Recognition (URGR) problem by aiming for a recognition distance of up to 25 meters and in the context of HRI. We propose the URGR framework, a novel deep-learning, using solely a simple RGB camera. Gesture inference is based on a single image. First, a novel super-resolution model termed High-Quality Network (HQ-Net) uses a set of self-attention and convolutional layers to enhance the low-resolution image of the user. Then, we propose a novel URGR classifier termed Graph Vision Transformer (GViT) which takes the enhanced image as input. GViT combines the benefits of a Graph Convolutional Network (GCN) and a modified Vision Transformer (ViT). Evaluation of the proposed framework over diverse test data yields a high recognition rate of 98.1%. The framework has also exhibited superior performance compared to human recognition in ultra-range distances. With the framework, we analyze and demonstrate the performance of an autonomous quadruped robot directed by human gestures in complex ultra-range indoor and outdoor environments, acquiring 96% recognition rate on average.

==> GVIT.tex <==
\subsection{Gestures Recognition in Long Range }
\label{sec:Long}

Gestures recognition encompasses a set of methodologies and algorithms designed to identify and interpret human gestures depicted within images. As discussed in Sections \ref{sec:introduction}-\ref{sec:relatedwork}, state-of-the-art approaches for gesture recognition are designed to identify human gestures in close proximity of up to 5 meters. Hence, given a quality improved image $\hve{I}$ taken from a distance of up to 25 meters, our proposed Graph-Vision Transformer (\gv\!\!) will output a solution to \ref{eq:P(O)}. 

As previously discussed, the greater the distance between the user and the camera, the more challenging it becomes for the model to accurately discern the executed gesture. This is primarily attributed to the substantial presence of background noise in such scenarios. In order to eliminate the influence of the background noise, user crop-out and quality improvement are exerted. Hence, for training, dataset $\mathcal{H}$ is pre-processed such that each image $\ve{I}_i\in\mathcal{H}$ is cropped (with YOLOv3) around the recognized user while maintaining the same image proportion as in Section \ref{sec:preproc}. Then, the cropped image is passed through the \hq for quality improvement yielding a modified training dataset $\bar{\mathcal{H}}=\{(\bve{I}_i,o_i, d_i)\}_{i=1}^N$ where $\hve{I}_i$ is the processed image.

The \gv model combines the power of Graph Convolutional Networks (GCN) \cite{Ullah2019} with the expressiveness of a modified Vision Transformers (ViT) \cite{dosovitskiy2020image}. Thus, it could effectively process and analyze structured data, such as images, with inherent graph-like relationships while leveraging the self-attention mechanism of ViT in order to capture fine-grained visual features. We briefly present the notion of these two models following with a discussion on GViT.


% ===========================

\subsubsection{GCN} A graph can represent relationships between pixels or image regions, allowing the model to capture spatial dependencies within the image. In graph representation, we can think of an image as a graph, where nodes represent pixels or regions, and edges represent connections or relationships between them. For example, each pixel can be a node, and edges can represent the spatial adjacency of pixels. The core of a GCN is the graph convolutional layer. In this layer, each node aggregates information from its neighboring nodes, considering both the node's own features and the features of its neighbors. This aggregation is performed through a weighted sum:
\begin{align}
h_i^{(l+1)} = \sigma \left( \sum_{j \in N(i)} \frac{1}{c_{ij}} W^l h_j^l \right)
\end{align}
Where $\mathbf{h_i^{(l+1)}}$ is the updated feature representation of node i in layer (l+1). $\mathbf{N(i)}$ represents the set of neighboring nodes of node i, $\mathbf{c_{ij}}$ represents the normalization term, the learnable weight matrix defined as $\mathbf{W^l}$ parameter and $\mathbf{h_j^l}$ is the feature representation of a neighboring node j in layer l.

The GCN has emerged as a versatile and powerful tool for image processing, offering distinct advantages over traditional Convolutional Neural Networks (CNNs). In the realm of image analysis, GCN utilize a graph-based structure to model intricate relationships among image elements, yielding significant benefits. Moreover, GCN has the ability to capture long-range dependencies and relationships between non-adjacent pixels and it can model non-local relationships in the data. Furthermore, GCN can adapt more naturally to complex structures such as irregular grid-like images and have fewer parameters compared to traditional CNNs, making them more memory-efficient and easier to train on datasets.

In the context of human gesture classification, GCNs can be used to effectively capture the spatial and temporal relationships between different body parts, as well as the contextual information of the surrounding environment. This allows GCNs to learn more robust and discriminative features for gesture recognition, leading to improved performance on challenging datasets.
component is responsible for modeling the underlying graph structure within the input data. It takes the raw image data $\ve{X}$ that serves as the initial feature representation and edge indices $\ve{E}$ that based on the dimensions of the input image. These indices define connections between nodes in the graph. The choice of these edge indices depends on the specific problem and how you want to capture relationships between elements in the image.




\subsubsection{ViT} The Vision Transformer (ViT) represents a novel approach to image recognition that deviates from the traditional Convolutional Neural Networks (CNNs).
The key steps in a Vision Transformer model begin with patch extraction, where input images are divided into non-overlapping patches, each treated as a sequence of feature vectors. To introduce spatial information, positional encodings are added to the patch embeddings. The core of ViT lies in its stack of transformer encoder layers, each containing multi-head self-attention for capturing long-range dependencies and feed-forward neural networks for feature transformation. This hierarchical approach, along with global average pooling and a classification head, is very beneficial for complex tasks like human gesture recognition. 
The self-attention mechanism is a crucial component, which calculates the importance of each patch with respect to others using the softmax function. In the self-attention mechanism equation, there are three key matrices come into play: $\mathbf{Q}$ (queries), $\mathbf{K}$ (keys), and $\mathbf{V}$ (values) depicted as follows:

\begin{align}
\text{Attention}(\mathbf{Q}, \mathbf{K}, \mathbf{V}) = \text{softmax}\left(\frac{\mathbf{Q} \mathbf{K}^T}{\sqrt{d_k}}\right) \mathbf{V}
\end{align}

These matrices are fundamental in the self-attention mechanism, where queries and keys determine the relationships and similarity with values. The Softmax function is applied to the result of the inner product between queries and keys, yielding attention scores that represent the importance of each value. The square root of $d_k$ is used as a scaling factor to ensure numerical stability. 
After self-attention, the output is passed through a position-wise feed-forward neural network: 

\begin{align}
\text{FFN}(x) = \text{ReLU}(W_2\text{ReLU}(W_1x + b_1) + b_2)
\end{align}
Where the $\mathbf{W}_1$, $\mathbf{b}_1$, $\mathbf{W}_2$ and $\mathbf{b}_2$ are learnable weights and biases.

The ViT model offers several advantages in image recognition, first is modeling long-range dependencies and non-local relationships, then capturing the intricate spatial and temporal relationships among different body parts. Moreover, ViT is adaptable to diverse data structures, including irregular grids, providing flexibility in analyzing complex image content.
% ===========================


\subsubsection{GViT} The integration of GCN and ViT in the GVIT model enables it to effectively model both local and global dependencies within structured data, making it highly versatile for a wide range of applications, including object recognition and more. We demonstrate the effectiveness of the GVIT architecture through experiments and evaluations on relevant datasets, showcasing its ability to achieve state-of-the-art results in tasks such as classifying human gestures in both short-term and long-term contexts.

First, we adjust the input image for the GCN model, and we convert the images into a graph-like structure. We start by calculating the node index for a given pixel position (i, j) in the image, and iterate through the pixels of the image using nested loops (i and j). For each pixel, we find its corresponding node index. Then, we iterate through the neighboring pixels (including diagonals) to establish edges between the current pixel's node and its neighbors, creating graph connectivity. We employ a function \(\mathcal{F}\) that generates edge indices \(\mathbf{E}\) based on the dimensions of the input data. These edge indices define the connections between nodes in the graph, facilitating the propagation of information: \(\mathbf{E} = \mathcal{F}(\text{Image Dimensions})\).
We used this data as input for the GCN model, this data is a critical component for the GCN, It defines the connectivity pattern of the graph, indicating which pixels are connected to each other in the image and used to compute graph convolutions, which allow the GCN to propagate information from neighboring pixels and capture dependencies in the image. 

Second, we propagate the data into two graph convolutional layers: 
\begin{align}
\ve{H}_1 &= \text{GLU}(\ve{X} \ve{W}_1 + \ve{b}_1) \\
\ve{H}_2 &= \text{GLU}(\ve{H}_1 \ve{W}_2  + \ve{b}_2)
\end{align}

Where $\mathbf{H}_1$ is the first graph convolutional layer and is computed by applying a GLU activation function to the product of the input data $\mathbf{X}$ and the weight matrix $\mathbf{W}_1$. The second graph convolutional layer $\mathbf{H}_2$, similarly computed using the output of the first layer ($\mathbf{H}_1$) and the second weight matrix $\mathbf{W}_2$. The weight matrices $\mathbf{W}_1$ and $\mathbf{W}_2$ play a crucial role in capturing and transforming the information within the graph structure. The Gated Linear Unit (GLU) activation function is designed to help capture complex patterns and dependencies in data by incorporating gating mechanisms, it combines information from two parallel linear transformations. The input data is passed through two linear transformations $\mathbf{W}_x$ and $\mathbf{V}_x$, and the GLU combines the information from both transformations by multiplying them element-wise
\( \text{GLU}(x) = (Wx) \cdot \sigma(Vx) \) where W and V are weight matrices, and x is the input. The key advantages of the GLU activation function in image classification tasks are capturing complex patterns, effective feature learning, and reducing overfitting.
We add Dropout between the GCN layers to help the model become more general and to mitigate overfitting.

Finally, we modified the ViT to capture complex visual patterns within the transformed graph data. It takes the output of GCN, denoted as \(\mathbf{H}^{(2)}\), as input, effectively replacing the patching part of the traditional ViT. The ViT model extracts meaningful features from the graph representation using self-attention mechanisms:
\[
\text{ViT Output} = \text{Self-Attention}(\mathbf{H}^{(2)})
\]
Following the self-attention step, the ViT Output is further processed through a Multilayer perceptron (MLP) head for classification into six classes.



==> q_8.tex <==
To reformulate equation 3, which represents the operation of the GCN, let's refine the variables, let's denote \( X \) as the input RGB image tensor, \( A \) as the adjacency matrix representing the spatial relationships between pixels, and \( H \) as the output feature map obtained after applying the GCN. Thus, the refined Formula 3 can be represented as:

\[
H = \sigma(\tilde{D}^{-\frac{1}{2}} \tilde{A} \tilde{D}^{-\frac{1}{2}} X W)
\]

Where \( \tilde{A} \) is the normalized adjacency matrix, \( \tilde{D} \) is the degree matrix
which is a diagonal matrix containing the sum of weights of the nodes in a graph, the normalization of the degree matrix scales the adjacency matrix such that each row and column is normalized by the square root of the corresponding node degree, helps to mitigate the effects of varying node degrees and improves the stability and performance of the GCN. 
, \( W \) is the weight matrix of the GCN layer, and \( \sigma \) denotes the activation function.

The input RGB image tensor is first transformed into a graph structure, where nodes represent pixels and edges represent spatial relationships. Then, the GCN layer utilizes this graph structure, along with the weight matrix \( W \), to perform convolutional operations on the input image. This process enables the GCN to capture spatial dependencies and extract features from the RGB image data.
\\

In the proposed Graph Convolutional Network (GCN) architecture, every pixel within the image is denoted as a node within a graph structure. By considering the dimensions of the input image, an edge index tensor is constructed to establish connections between nodes, forming a graphical depiction of the image. Each pixel functions as a node, and edges are established between adjacent pixels within a predefined spatial proximity.

This functionality can be mathematically described through the concept of an adjacency matrix, denoted here as $A$. Each element $A_{i,j}$ of this matrix represents the connection strength between nodes $i$ and $j$, corresponding to individual pixels in the image. 
\[
A_{i,j} = \begin{cases}
1 & \text{if } |i_x - j_x| \leq 1 \text{ and } |i_y - j_y| \leq 1 \text{ and } i \neq j \\
0 & \text{otherwise}
\end{cases}
\]
where $i$ and $j$ represent the node indices (pixel locations). This formulation describes the construction of the image graph and its corresponding adjacency matrix. In our example the number of edge indexes for 224x224 pixel image is 398724 and the total number of nodes is 50,176 nodes.

